Insider Purchases Far Below the 52-Week High: Decomposing the Disclosure Reaction in Microcap Equities

Purchases reported under transaction code P on SEC Form 4 by insiders of U.S. equities with an estimated filing-date capitalization of USD 30 million to USD 500 million (13,534 lines, 1,192 issuers, 2018-2024) are followed by a first-day abnormal return that rises steeply with the stock's distance below its 52-week high: 4.13% in the quintile farthest below the high against 0.86% nearest it (two-way clustered t = 9.77); random non-event days of the same issuers show 0.14%. Five tests with decision rules fixed in advance characterize the gradient. Most of it is scale: the beaten-down stocks are 3.10 times as volatile, and with a full set of controls the raw gap fails its pre-specified bar (0.94 points, t = 2.11). Per unit of the stock's own volatility the reaction is 2.51 times as large far below the high (t = 7.49), 1.28 to 3.50 on other estimators, though a variance-weighted slope shows none. The gradient is larger than for insider sales by the same issuers and for positive earnings surprises as a class; against the strongest surprises the difference is imprecise. Dropping purchases with a concurrent 8-K leaves the raw gradient intact (t = 7.13), but the per-risk gradient no longer clears the controls (t = 2.52). The reaction runs for two to three sessions; the 29-day drift is imprecise (two-way t = 1.70) and a calendar-time portfolio that skips the first day earns no significant alpha. The analysis quantifies sensitivity to price adjustment and benchmark specification: mixing price bases misassigns run-up buckets, and carrying the estimation-window intercept supplies 57% of the 30-day gradient under that benchmark. A gradient-boosting classifier (test AUC 0.676) is indistinguishable from logistic regression. A separate large-cap extension schedules USD 29,075,559 a year of buyer-cluster flow but fails every matched-comparison gate.

==> outputs/table_classification_delong.tex <==
XGBoost $-$ random forest (full) & 0.002 & [$-$0.012, 0.017] & 0.008 & 0.795 & 0.42 & 0.671 \\
XGBoost $-$ logistic regression (full) & 0.023 & [$-$0.003, 0.051] & 0.015 & 0.113 & 2.44 & 0.015 \\
Random forest $-$ logistic regression (full) & 0.021 & [$-$0.004, 0.047] & 0.013 & 0.103 & 2.42 & 0.015 \\
XGBoost $-$ random forest (base) & 0.007 & [$-$0.012, 0.030] & 0.011 & 0.516 & 1.28 & 0.202 \\
XGBoost full $-$ XGBoost base & $-$0.006 & [$-$0.021, 0.008] & 0.008 & 0.429 & $-$1.26 & 0.207 \\
XGBoost full: CV rounds $-$ validation-based early stopping & 0.001 & [$-$0.012, 0.012] & 0.006 & 0.919 & 0.18 & 0.859 \\
XGBoost base: CV rounds $-$ validation-based early stopping & $-$0.001 & [$-$0.007, 0.005] & 0.003 & 0.724 & $-$0.44 & 0.663 \\
\bottomrule


==> outputs/table_classification_perf.tex <==
XGBoost & Full & 0.676 & 0.628--0.714 & 0.419 & 0.500 & 0.510 & 0.094 & 0.159 & 98 \\
\quad optimized &  &  &  &  & 0.184 & 0.338 & 0.765 & 0.469 & 1,205 \\
Random forest & Full & 0.674 & 0.621--0.718 & 0.419 & 0.500 & 0.561 & 0.120 & 0.198 & 114 \\
\quad optimized &  &  &  &  & 0.257 & 0.367 & 0.639 & 0.466 & 926 \\
Logistic regression & Full & 0.653 & 0.600--0.700 & 0.390 & 0.500 & 0.519 & 0.130 & 0.208 & 133 \\
\quad optimized &  &  &  &  & 0.245 & 0.345 & 0.590 & 0.436 & 910 \\
\midrule
XGBoost & Base & 0.682 & 0.632--0.723 & 0.421 & 0.500 & 0.567 & 0.064 & 0.115 & 60 \\
\quad optimized &  &  &  &  & 0.210 & 0.350 & 0.767 & 0.481 & 1,165 \\
Random forest & Base & 0.675 & 0.626--0.716 & 0.408 & 0.500 & 0.574 & 0.117 & 0.194 & 108 \\
\quad optimized &  &  &  &  & 0.281 & 0.375 & 0.594 & 0.460 & 843 \\
Logistic regression & Base & 0.655 & 0.599--0.703 & 0.386 & 0.500 & 0.556 & 0.139 & 0.223 & 133 \\
\quad optimized &  &  &  &  & 0.221 & 0.336 & 0.650 & 0.443 & 1,030 \\
\midrule
XGBoost (validation-based early stopping) & Full & 0.675 & 0.628--0.716 & 0.417 & 0.500 & 0.510 & 0.049 & 0.089 & 51 \\
\quad optimized &  &  &  &  & 0.220 & 0.350 & 0.756 & 0.478 & 1,150 \\
XGBoost (validation-based early stopping) & Base & 0.683 & 0.635--0.724 & 0.417 & 0.500 & 0.478 & 0.021 & 0.040 & 23 \\
\quad optimized &  &  &  &  & 0.240 & 0.356 & 0.739 & 0.480 & 1,104 \\
\bottomrule


==> outputs/table_economics_calendar.tex <==
All filings, 2018--2024 & 1,787 & 227 & 2.10\% & 5.28 & 0.95 & 1.16 & 0.41 & 2.21\% & 5.50 \\
All 2024 filings & 281 & 217 & 2.04\% & 2.37 & 0.90 & 1.17 & 0.33 & 1.99\% & 2.35 \\
2024, model-flagged & 281 & 129 & 3.48\% & 1.89 & 0.93 & 1.33 & 0.02 & 3.43\% & 1.87 \\
2024, rejected & 281 & 88 & $-$0.13\% & $-$0.22 & 0.87 & 0.84 & 0.79 & $-$0.13\% & $-$0.20 \\
Deviation $\leq$ 0\% & 1,785 & 102 & 2.24\% & 3.96 & 0.97 & 1.15 & 0.46 & 2.37\% & 4.15 \\
Deviation $>$ 10\% & 1,785 & 22 & 3.16\% & 2.99 & 1.07 & 1.24 & 0.14 & 3.66\% & 3.45 \\
CEO & 1,780 & 41 & 2.13\% & 3.58 & 0.94 & 1.25 & 0.29 & 2.35\% & 3.89 \\
CFO & 1,753 & 16 & 4.02\% & 5.56 & 0.96 & 1.30 & 0.31 & 4.12\% & 5.68 \\
Other officer & 1,780 & 49 & 2.58\% & 4.71 & 0.99 & 1.19 & 0.43 & 2.74\% & 4.93 \\
Director & 1,785 & 120 & 1.85\% & 4.16 & 0.95 & 1.12 & 0.49 & 1.90\% & 4.31 \\
10\% owner & 1,787 & 52 & 2.25\% & 2.93 & 0.86 & 1.26 & 0.18 & 2.33\% & 2.94 \\
2024, flagged minus rejected & 281 & 217 & 3.62\% & 1.78 & 0.06 & 0.49 & $-$0.77 & 3.56\% & 1.77 \\
\bottomrule


==> outputs/table_economics_cost.tex <==
Full sample, all filings & 13,534 & 3.6\% & [2.8\%, 4.4\%] & 2.6\% & 1.6\% & 0.6\% & $-$1.4\% \\
Deviation bucket $\leq$ 0\% & 6,067 & 4.0\% & [3.0\%, 5.4\%] & 3.0\% & 2.0\% & 1.0\% & $-$1.0\% \\
Deviation bucket 0\% -- 3\% & 3,733 & 2.5\% & [1.7\%, 3.3\%] & 1.5\% & 0.5\% & $-$0.5\% & $-$2.5\% \\
Deviation bucket 3\% -- 5\% & 1,164 & 3.3\% & [1.8\%, 4.9\%] & 2.3\% & 1.3\% & 0.3\% & $-$1.7\% \\
Deviation bucket 5\% -- 10\% & 1,283 & 2.6\% & [1.0\%, 4.5\%] & 1.6\% & 0.6\% & $-$0.4\% & $-$2.4\% \\
Deviation bucket $>$ 10\% & 1,287 & 6.1\% & [3.7\%, 8.6\%] & 5.1\% & 4.1\% & 3.1\% & 1.1\% \\
2024, all filings (buy-all) & 2,033 & 3.3\% & [1.6\%, 5.2\%] & 2.3\% & 1.3\% & 0.3\% & $-$1.7\% \\
2024, model-flagged & 1,205 & 5.2\% & [2.5\%, 8.0\%] & 4.2\% & 3.2\% & 2.2\% & 0.2\% \\
2024, rejected & 828 & 0.7\% & [$-$0.9\%, 2.5\%] & $-$0.3\% & $-$1.3\% & $-$2.3\% & $-$4.3\% \\
2024, deviation $>$ 10\% & 213 & 5.3\% & [$-$0.1\%, 10.9\%] & 4.3\% & 3.3\% & 2.3\% & 0.3\% \\
\bottomrule


==> outputs/table_importance_full.tex <==
1 & \texttt{volatility\_30d} & 0.187 & 0.285 (1) & 0.087 (5) & 0.093 (4) & 0.371 & 0.303 (1) \\
2 & \texttt{return\_21d} & 0.084 & 0.121 (3) & 0.083 (7) & 0.054 (7) & 0.096 & 0.078 (4) \\
3 & \texttt{return\_5d} & 0.067 & 0.067 (6) & 0.057 (8) & 0.056 (6) & 0.048 & 0.039 (6) \\
4 & \texttt{pct\_from\_52w\_high} & 0.066 & 0.128 (2) & 0.111 (1) & 0.073 (5) & 0.215 & 0.176 (2) \\
5 & \texttt{pre\_close} & 0.044 & 0.006 (17) & 0.008 (19) & 0.093 (3) & 0.024 & 0.019 (13) \\
6 & \texttt{pct\_from\_52w\_low} & 0.044 & 0.080 (4) & 0.104 (2) & 0.042 (10) & 0.103 & 0.084 (3) \\
7 & \texttt{return\_mtd} & 0.043 & 0.068 (5) & 0.090 (3) & 0.043 (9) & 0.069 & 0.056 (5) \\
8 & \texttt{n\_prior\_purchases\_365d} & 0.043 & 0.011 (15) & 0.015 (16) & 0.039 (11) & 0.018 & 0.014 (14) \\
9 & \texttt{cmp\_routine} & 0.034 & 0.015 (12) & 0.024 (13) & 0.033 (12) & 0.034 & 0.028 (10) \\
10 & \texttt{addv\_30d} & 0.034 & 0.051 (8) & 0.087 (6) & 0.029 (13) & 0.036 & 0.030 (9) \\
11 & \texttt{is\_biotech} & 0.034 & 0.002 (23) & 0.003 (23) & 0.099 (2) & 0.007 & 0.006 (18) \\
12 & \texttt{market\_cap\_pit} & 0.033 & 0.052 (7) & 0.090 (4) & 0.021 (17) & 0.047 & 0.039 (7) \\
13 & \texttt{pct\_of\_holdings} & 0.032 & 0.019 (11) & 0.034 (11) & 0.051 (8) & 0.038 & 0.031 (8) \\
14 & \texttt{transaction\_value} & 0.029 & 0.023 (9) & 0.045 (9) & 0.014 (18) & 0.032 & 0.026 (11) \\
15 & \texttt{days\_since\_last\_purchase} & 0.027 & 0.014 (13) & 0.028 (12) & 0.008 (21) & 0.015 & 0.012 (16) \\
16 & \texttt{n\_other\_insiders\_30d} & 0.027 & 0.012 (14) & 0.024 (14) & 0.008 (20) & 0.015 & 0.013 (15) \\
17 & \texttt{value\_vs\_avg\_ratio} & 0.027 & 0.020 (10) & 0.043 (10) & 0.025 (16) & 0.024 & 0.020 (12) \\
18 & \texttt{price\_deviation} & 0.027 & 0.010 (16) & 0.022 (15) & 0.027 (14) & 0.006 & 0.005 (19) \\
19 & \texttt{n\_purchases\_30d} & 0.026 & 0.004 (20) & 0.008 (20) & 0.144 (1) & 0.003 & 0.003 (22) \\
20 & \texttt{is\_other\_officer} & 0.025 & 0.002 (22) & 0.004 (22) & 0.004 (23) & 0.001 & 0.001 (23) \\
21 & \texttt{is\_director} & 0.023 & 0.004 (19) & 0.009 (18) & 0.013 (19) & 0.010 & 0.008 (17) \\
22 & \texttt{insider\_title\_score} & 0.018 & 0.002 (21) & 0.007 (21) & 0.026 (15) & 0.006 & 0.005 (20) \\
23 & \texttt{filing\_lag\_days} & 0.015 & 0.004 (18) & 0.015 (17) & 0.004 (22) & 0.004 & 0.003 (21) \\
24 & \texttt{is\_10pct\_owner} & 0.012 & 0.000 (24) & 0.001 (24) & 0.000 (24) & 0.000 & 0.000 (24) \\
-- & \texttt{is\_first\_purchase\_12m} & 0.000 & 0.000 (--) & 0.000 (--) & 0.000 (--) & 0.000 & 0.000 (--) \\
-- & \texttt{is\_ceo} & 0.000 & 0.000 (--) & 0.000 (--) & 0.000 (--) & 0.000 & 0.000 (--) \\
-- & \texttt{is\_cfo} & 0.000 & 0.000 (--) & 0.000 (--) & 0.000 (--) & 0.000 & 0.000 (--) \\
\bottomrule


==> outputs/table_mechanism_floor.tex <==
all & 13,534 & 100.0\% & 2,033 & 26.2\% & 0.676 & 0.676 & 6,067 & 1,287 & 4.0\% & 6.1\% & 2.1 & 1.60 & 2.62 & 27.2\% & 38.8\% & 4.88 \\
$\geq$ \$1 & 13,109 & 96.9\% & 1,933 & 25.3\% & 0.668 & 0.672 & 5,850 & 1,234 & 4.0\% & 5.9\% & 1.9 & 1.47 & 2.46 & 26.8\% & 38.7\% & 4.91 \\
$\geq$ \$2 & 11,855 & 87.6\% & 1,705 & 23.4\% & 0.668 & 0.678 & 5,290 & 1,019 & 2.8\% & 3.8\% & 1.0 & 0.79 & 1.26 & 24.3\% & 34.8\% & 4.09 \\
$\geq$ \$5 & 9,095 & 67.2\% & 1,327 & 18.5\% & 0.644 & 0.631 & 4,081 & 638 & 1.6\% & 1.3\% & $-$0.3 & $-$0.22 & $-$0.39 & 20.3\% & 29.5\% & 2.80 \\
\bottomrule


==> outputs/table_mechanism_quintiles.tex <==
Q1 & 2,707 & $-$77.0\% & 43.0\% & 25.2\% & 8.6\% & 5.5\% & 29.8\% & 1.19 & 13.7\% & 0.21 & 37.2\% \\
Q2 & 2,708 & $-$55.3\% & 35.1\% & 21.2\% & 5.2\% & 3.5\% & 25.0\% & 0.84 & 12.2\% & 0.18 & 31.7\% \\
Q3 & 2,705 & $-$40.4\% & 23.9\% & 19.5\% & 1.7\% & 0.8\% & 17.0\% & 0.68 & 10.4\% & 0.10 & 21.8\% \\
Q4 & 2,707 & $-$26.1\% & 17.0\% & 19.0\% & 0.7\% & $-$0.1\% & 16.5\% & 0.49 & 11.3\% & 0.02 & 16.0\% \\
Q5 & 2,707 & $-$10.4\% & 16.5\% & 11.3\% & 1.7\% & 0.5\% & 14.1\% & 0.41 & 11.7\% & 0.05 & 15.0\% \\
\bottomrule


==> outputs/table_mechanism_quintiles_v1.tex <==
Q1 & 2,707 & $-$77.0\% & $-$21.6 & 6.48 & 8.6\% & 15.1\% & 11.8\% & 43.0\% & 53.0\% & 17.7\% \\
Q2 & 2,708 & $-$55.3\% & $-$5.8 & 1.75 & 5.2\% & 6.9\% & 6.0\% & 35.1\% & 40.4\% & 20.0\% \\
Q3 & 2,705 & $-$40.4\% & 0.4 & $-$0.11 & 1.7\% & 1.6\% & 1.8\% & 23.9\% & 25.5\% & 21.0\% \\
Q4 & 2,707 & $-$26.1\% & 2.9 & $-$0.86 & 0.7\% & $-$0.1\% & $-$0.2\% & 17.0\% & 16.0\% & 20.3\% \\
Q5 & 2,707 & $-$10.4\% & 8.9 & $-$2.68 & 1.7\% & $-$0.9\% & $-$1.2\% & 16.5\% & 13.4\% & 16.7\% \\
\bottomrule


==> outputs/table_placebo_quintiles.tex <==
Q1 & 2,707 & 25,040 & 7.58 & 8.64\% & 1.47\% & 15.13\% & 9.05\% & 7.73\% & 0.71\% \\
Q2 & 2,708 & 22,679 & 1.02 & 5.18\% & $-$0.19\% & 6.93\% & 0.83\% & 4.43\% & $-$0.87\% \\
Q3 & 2,705 & 23,735 & $-$0.93 & 1.67\% & $-$0.91\% & 1.56\% & $-$1.84\% & 0.86\% & $-$1.25\% \\
Q4 & 2,707 & 31,470 & $-$2.29 & 0.72\% & $-$0.45\% & $-$0.14\% & $-$2.74\% & $-$0.35\% & $-$0.85\% \\
Q5 & 2,707 & 48,698 & $-$3.73 & 1.75\% & 0.19\% & $-$0.93\% & $-$3.54\% & 1.14\% & $-$0.35\% \\
\midrule
Q1 $-$ Q5 (pp) &  &  & 11.31 & 6.90 & 1.27 & 16.05 & 12.58 & 6.60 & 1.07 \\
\quad two-way $t$ &  &  & 28.27 & 3.15 & 0.95 & 7.59 & 9.27 & 2.93 & 0.63 \\
\midrule
Q1: event $-$ placebo (pp) &  &  &  &  & 7.18 &  & 6.08 &  & 7.02 \\
\quad two-way $t$ &  &  &  &  & 3.36 &  & 2.95 &  & 3.61 \\
Q1: placebo / event &  &  &  &  & 0.17 &  & 0.60 &  & 0.09 \\
\bottomrule


==> outputs/table_reaction_calendar.tex <==
Q1 (farthest below the high) & EW & $t_0{+}1 \ldots t_0{+}30$ & 1,758 & 46 & 4.26\% & 3.41 & 1.16 & 1.65 & 0.11 & $-$0.39 & 4.18\% & 3.31 \\
 & EW & $t_0{+}2 \ldots t_0{+}31$ & 1,758 & 46 & 0.95\% & 0.79 & 1.16 & 1.64 & 0.11 & $-$0.38 & 0.87\% & 0.72 \\
\midrule
 & VW & $t_0{+}1 \ldots t_0{+}30$ & 1,758 & 46 & 4.24\% & 3.34 & 1.26 & 1.64 & 0.15 & $-$0.41 & 4.15\% & 3.24 \\
 & VW & $t_0{+}2 \ldots t_0{+}31$ & 1,758 & 46 & 1.01\% & 0.82 & 1.23 & 1.61 & 0.13 & $-$0.41 & 0.93\% & 0.74 \\
\midrule
Q5 (nearest the high) & EW & $t_0{+}1 \ldots t_0{+}30$ & 1,787 & 45 & 1.91\% & 3.98 & 0.78 & 0.67 & 0.43 & 0.18 & 1.96\% & 4.13 \\
 & EW & $t_0{+}2 \ldots t_0{+}31$ & 1,787 & 45 & 1.07\% & 2.38 & 0.77 & 0.67 & 0.41 & 0.20 & 1.12\% & 2.50 \\
\midrule
 & VW & $t_0{+}1 \ldots t_0{+}30$ & 1,787 & 45 & 1.16\% & 2.62 & 0.77 & 0.74 & 0.46 & 0.20 & 1.21\% & 2.77 \\
 & VW & $t_0{+}2 \ldots t_0{+}31$ & 1,787 & 45 & 0.48\% & 1.12 & 0.76 & 0.73 & 0.45 & 0.21 & 0.53\% & 1.26 \\
\midrule
All filings & EW & $t_0{+}1 \ldots t_0{+}30$ & 1,787 & 227 & 2.14\% & 5.54 & 0.94 & 1.10 & 0.35 & $-$0.15 & 2.10\% & 5.28 \\
 & EW & $t_0{+}2 \ldots t_0{+}31$ & 1,787 & 227 & 0.68\% & 1.78 & 0.93 & 1.10 & 0.35 & $-$0.15 & 0.64\% & 1.63 \\
\midrule
 & VW & $t_0{+}1 \ldots t_0{+}30$ & 1,787 & 227 & 1.81\% & 5.32 & 0.95 & 1.11 & 0.43 & $-$0.14 & 1.77\% & 5.03 \\
 & VW & $t_0{+}2 \ldots t_0{+}31$ & 1,787 & 227 & 0.53\% & 1.60 & 0.95 & 1.10 & 0.43 & $-$0.15 & 0.50\% & 1.44 \\
\midrule
Q1 $-$ Q5 & EW & $t_0{+}1 \ldots t_0{+}30$ & 1,758 & 28 & 2.30\% & 1.74 & 0.39 & 0.98 & $-$0.32 & $-$0.57 & 2.18\% & 1.64 \\
 & EW & $t_0{+}2 \ldots t_0{+}31$ & 1,758 & 28 & $-$0.17\% & $-$0.14 & 0.39 & 0.97 & $-$0.29 & $-$0.59 & $-$0.29\% & $-$0.23 \\
\midrule
 & VW & $t_0{+}1 \ldots t_0{+}30$ & 1,758 & 28 & 3.04\% & 2.22 & 0.49 & 0.91 & $-$0.31 & $-$0.61 & 2.91\% & 2.11 \\
 & VW & $t_0{+}2 \ldots t_0{+}31$ & 1,758 & 28 & 0.48\% & 0.36 & 0.47 & 0.88 & $-$0.32 & $-$0.62 & 0.35\% & 0.26 \\
\bottomrule


==> outputs/table_reaction_floor.tex <==
\multicolumn{10}{l}{\emph{Price $\geq$ \$5 ($N$ = 9,095, 67.2\% of the sample)}} \\
\quad Q1 & 725 & 4.17\% & 7.16 & 7.98 & 2.09\% & 1.64 & 1.23 & 6.26\% & 0.67 \\
\quad Q5 & 2,474 & 0.57\% & 5.93 & 5.44 & 0.01\% & 0.02 & 0.02 & 0.58\% & 0.99 \\
\quad Q1 $-$ Q5 (pp) &  & 3.60 & 6.08 & 6.57 & 2.09 & 1.58 & 1.22 & 5.69 & -- \\
\multicolumn{10}{l}{\quad Q1 in calendar time (EW, FF3+UMD $\alpha$ per month, NW $t$): with day 1 3.30\% ($t$ = 1.71), skipping day 1 0.96\% ($t$ = 0.56); 1,638 days, 13.3 positions on average} \\
\midrule
\multicolumn{10}{l}{\emph{Price $\geq$ \$5 and ADDV $\geq$ \$1M ($N$ = 4,131, 30.5\% of the sample)}} \\
\quad Q1 & 546 & 4.73\% & 6.65 & 7.86 & 1.70\% & 1.05 & 0.70 & 6.43\% & 0.74 \\
\quad Q5 & 767 & 1.09\% & 5.27 & 5.23 & 0.44\% & 0.53 & 0.51 & 1.53\% & 0.72 \\
\quad Q1 $-$ Q5 (pp) &  & 3.64 & 4.88 & 5.65 & 1.27 & 0.71 & 0.50 & 4.90 & -- \\
\multicolumn{10}{l}{\quad Q1 in calendar time (EW, FF3+UMD $\alpha$ per month, NW $t$): with day 1 2.47\% ($t$ = 1.26), skipping day 1 $-$0.28\% ($t$ = $-$0.16); 1,571 days, 10.4 positions on average} \\
\bottomrule


==> outputs/table_reaction_quintiles.tex <==
Q1 & 2,707 & $-$77.0\% & 2.60\% & 4.13\% & 13.19 & 4.52\% & 3.62 & 7.26\% & 8.64\% & 6.64 & 0.48 \\
Q2 & 2,708 & $-$55.3\% & 2.23\% & 2.42\% & 10.10 & 2.76\% & 3.22 & 2.97\% & 5.18\% & 5.76 & 0.47 \\
Q3 & 2,705 & $-$40.4\% & 1.61\% & 1.39\% & 11.72 & 0.28\% & 0.53 & 0.84\% & 1.67\% & 3.06 & 0.83 \\
Q4 & 2,707 & $-$26.1\% & 1.03\% & 0.79\% & 8.15 & $-$0.07\% & $-$0.15 & 0.75\% & 0.72\% & 1.40 & 1.10 \\
Q5 & 2,707 & $-$10.4\% & 0.90\% & 0.86\% & 6.75 & 0.88\% & 1.87 & 1.77\% & 1.75\% & 3.45 & 0.49 \\
\midrule
Q1 $-$ Q5 &  &  & 1.70 & 3.27 & 9.55 & 3.63 & 2.73 & 5.50 & 6.90 & 4.92 & -- \\
\bottomrule


==> outputs/table_reaction_timing.tex <==
Filed before the 16:00 ET close: all & 5,408 & 1.57\% & 11.98 & 0.58\% & 5.60 & 0.30\% & 4.75 & 0.21\% & 2.42 & 1.42\% & 2.00\% \\
\quad Q1 & 803 & 2.60\% & 5.70 & 1.74\% & 3.16 & 0.61\% & 1.77 & 0.84\% & 2.04 & 4.00\% & 5.74\% \\
\quad Q5 & 1,332 & 0.90\% & 6.40 & 0.33\% & 2.90 & 0.17\% & 3.46 & 0.13\% & 1.23 & 1.32\% & 1.65\% \\
\quad Q1 $-$ Q5 &  & 1.70 & 3.53 & 1.41 & 2.51 & 0.44 & 1.27 & 0.72 & 1.69 & 2.67 & 4.08 \\
\midrule
Filed after the close: all & 8,126 & 0.17\% & 1.92 & 2.81\% & 18.92 & 1.96\% & 20.12 & 0.76\% & 7.37 & 1.84\% & 4.65\% \\
\quad Q1 & 1,904 & 0.14\% & 0.48 & 5.14\% & 14.89 & 3.27\% & 15.31 & 1.68\% & 5.72 & 4.74\% & 9.87\% \\
\quad Q5 & 1,375 & 0.58\% & 3.97 & 1.38\% & 6.94 & 0.91\% & 7.20 & 0.43\% & 2.31 & 0.46\% & 1.84\% \\
\quad Q1 $-$ Q5 &  & $-$0.45 & $-$1.43 & 3.76 & 9.34 & 2.35 & 9.50 & 1.24 & 3.55 & 4.28 & 8.04 \\
\bottomrule


==> outputs/table_robustness_rolling.tex <==
2020 & 2018 & 2019 & 1,122 & 2,286 & 35.6\% & 298 & 0.623 & [0.584, 0.660] & 0.673 & 0.600 & 0.551 \\
2021 & 2018--2019 & 2020 & 2,527 & 1,715 & 22.5\% & 2 & 0.626 & [0.571, 0.678] & 0.698 & 0.697 & 0.426 \\
2022 & 2018--2020 & 2021 & 4,813 & 2,516 & 25.4\% & 41 & 0.660 & [0.616, 0.702] & 0.674 & 0.673 & 0.463 \\
2023 & 2018--2021 & 2022 & 6,528 & 2,457 & 27.3\% & 22 & 0.688 & [0.649, 0.729] & 0.695 & 0.688 & 0.491 \\
2024 & 2018--2022 & 2023 & 9,044 & 2,033 & 26.2\% & 26 & 0.676 & [0.628, 0.714] & 0.674 & 0.653 & 0.469 \\
\bottomrule


==> outputs/table_robustness_tails_model.tex <==
Baseline ($CAR_{30}$, FF3 betas only) & 2,033 & 26.2\% & 0.676 & [0.628, 0.714] & 5.15\% & 0.71\% & 4.45 & 2.85 \\
Excluding $|CAR_{30}| > 1$ & 2,016 & 25.5\% & 0.668 & [0.620, 0.712] & 3.54\% & 0.71\% & 2.84 & 2.02 \\
$CAR_{30}$ winsorized 1/99 & 2,033 & 26.2\% & 0.676 & [0.628, 0.714] & 4.66\% & 0.68\% & 3.98 & 2.80 \\
$BHAR_{30}$ & 2,033 & 24.2\% & 0.651 & [0.600, 0.694] & 4.66\% & 0.66\% & 4.00 & 2.53 \\
$CAR_{30}$, timing-adjusted & 2,033 & 23.2\% & 0.669 & [0.617, 0.711] & 2.36\% & 0.39\% & 1.97 & 1.28 \\
$CAR_{30}^{\alpha}$, intercept included & 2,033 & 27.8\% & 0.658 & [0.612, 0.697] & 5.31\% & 1.11\% & 4.20 & 2.51 \\
\bottomrule


==> outputs/table_roles_car.tex <==
All lines & 13,534 & 100.0\% & 3.6\% & 1.3\% & 27.1\% & -- & -- \\
\midrule
CEO & 2,406 & 17.8\% & 3.4\% & 1.3\% & 28.1\% & $-$0.36 & $-$0.50 \\
CFO & 909 & 6.7\% & 6.0\% & 3.2\% & 35.8\% & 2.88 & 3.50 \\
Other officer & 2,924 & 21.6\% & 4.9\% & 1.8\% & 29.4\% & 2.28 & 3.69 \\
Any officer title & 4,707 & 34.8\% & 4.5\% & 1.7\% & 30.3\% & 2.25 & 3.62 \\
Director (any) & 7,136 & 52.7\% & 3.4\% & 1.3\% & 25.2\% & $-$0.76 & $-$1.23 \\
Director only (no officer title) & 6,700 & 49.5\% & 3.4\% & 1.3\% & 25.0\% & $-$0.73 & $-$1.18 \\
Director \& officer & 436 & 3.2\% & 3.4\% & 1.8\% & 28.0\% & $-$0.14 & $-$0.16 \\
10\% beneficial owner & 3,082 & 22.8\% & 2.7\% & 0.1\% & 27.0\% & $-$1.34 & $-$2.40 \\
No role flag & 339 & 2.5\% & 2.5\% & 1.8\% & 29.5\% & $-$0.53 & $-$1.03 \\
\bottomrule


==> outputs/table_runup_artefact.tex <==
$\leq$ 0\% & 7,951 & 3.3\% & 22.7\% & 6,067 & 4.0\% & 27.2\% & 10,787 & 2.3\% & 22.6\% \\
0\% -- 3\% & 1,516 & 4.3\% & 30.5\% & 3,733 & 2.5\% & 22.4\% & 1,820 & 4.7\% & 31.2\% \\
3\% -- 5\% & 555 & 5.9\% & 33.0\% & 1,164 & 3.3\% & 27.0\% & 662 & 4.4\% & 34.9\% \\
5\% -- 10\% & 684 & 4.1\% & 34.5\% & 1,283 & 2.6\% & 29.1\% & 793 & 4.8\% & 36.1\% \\
$>$ 10\% & 2,828 & 3.5\% & 34.8\% & 1,287 & 6.1\% & 38.8\% & 2,998 & 6.3\% & 36.7\% \\
\midrule
$>$ 10\% minus $\leq$ 0\% (pp) & 0.2 & Welch $t$ = 0.33 & cl.\ $t$ = 0.17 & 2.1 & Welch $t$ = 2.62 & cl.\ $t$ = 1.60 & 4.0 & Welch $t$ = 5.13 & cl.\ $t$ = 2.59 \\
Pr(CAR $>$ 10\%) difference (pp) & 12.1 &  & cl.\ $t$ = 6.33 & 11.6 &  & cl.\ $t$ = 4.88 & 14.1 &  & cl.\ $t$ = 5.68 \\
\bottomrule


==> outputs/table_runup_buckets.tex <==
$\leq$ 0\% & 6,067 & 1,009 & 4.0\% & [2.8\%, 5.3\%] & 1.4\% & 3.3\% & 27.2\% & 0.58 & 8.8\% & $-$41.8\% \\
0\% -- 3\% & 3,733 & 773 & 2.5\% & [1.6\%, 3.3\%] & 1.1\% & 2.1\% & 22.4\% & 0.47 & 7.2\% & $-$33.2\% \\
3\% -- 5\% & 1,164 & 516 & 3.3\% & [1.8\%, 4.8\%] & 1.1\% & 2.7\% & 27.0\% & 0.61 & 9.5\% & $-$41.8\% \\
5\% -- 10\% & 1,283 & 576 & 2.6\% & [1.0\%, 4.3\%] & 0.0\% & 2.2\% & 29.1\% & 0.74 & 11.1\% & $-$45.5\% \\
$>$ 10\% & 1,287 & 487 & 6.1\% & [3.7\%, 8.5\%] & 3.1\% & 5.8\% & 38.8\% & 0.94 & 14.5\% & $-$50.2\% \\
\midrule
\quad 10\% -- 25\% & 976 & 436 & 7.2\% & [4.8\%, 9.6\%] & 4.0\% & 6.9\% & 40.1\% & 0.91 & 13.4\% & $-$51.4\% \\
\quad 25\% -- 50\% & 211 & 127 & 6.6\% & [1.7\%, 11.6\%] & 3.9\% & 6.2\% & 42.2\% & 1.19 & 17.9\% & $-$49.3\% \\
\quad 50\% -- 100\% & 100 & 39 & $-$5.3\% & [$-$14.9\%, 4.4\%] & $-$11.7\% & $-$5.3\% & 19.0\% & 0.49 & 15.6\% & $-$29.3\% \\
\bottomrule


==> outputs/table_runup_doublesort.tex <==
Q1 (furthest from high) [$-$100\%, $-$65\%] & 9.7\% (1,285) & 8.3\% (402) & $-$1.3 & $-$0.42 \\
Q2 [$-$65\%, $-$47\%] & 6.6\% (1,238) & 5.2\% (285) & $-$1.4 & $-$0.43 \\
Q3 [$-$47\%, $-$33\%] & 1.8\% (1,245) & 5.4\% (210) & 3.6 & 1.72 \\
Q4 [$-$33\%, $-$19\%] & 0.6\% (1,216) & 2.0\% (166) & 1.4 & 0.44 \\
Q5 (nearest high) [$-$19\%, 0\%] & 0.8\% (1,083) & 7.0\% (224) & 6.2 & 2.26 \\
\midrule
All & 4.0\% (6,067) & 6.1\% (1,287) & 2.1 & 1.60 \\
\bottomrule


==> outputs/table_runup_regressions.tex <==
CAR$_{30}$ (pp) & 1.6 & 1.20 & 0.6 & 0.42 & $-$0.2 & $-$0.12 \\
CAR$_{30}$, 1/99 winsorized (pp) & 1.9 & 1.57 & 0.9 & 0.80 & 0.4 & 0.31 \\
1\{CAR$_{30} > 10\%$\}, LPM (pp) & 10.8 & 4.69 & 8.1 & 3.72 & 4.9 & 2.16 \\
1\{CAR$_{30} > 10\%$\}, logit (log-odds) & 0.50 & 4.89 & 0.40 & 3.90 & 0.24 & 2.21 \\
\bottomrule


==> outputs/table_runup_subsamples.tex <==
All lines & 6,067 & 1,287 & 4.0\% & 6.1\% & 2.1 & 2.62 & 1.60 & 27.2\% & 38.8\% \\
\multicolumn{10}{l}{\emph{By filing year}} \\
2018 & 522 & 62 & 2.6\% & $-$0.7\% & $-$3.3 & $-$1.21 & $-$1.46 & 22.8\% & 21.0\% \\
2019 & 593 & 119 & 4.3\% & 12.6\% & 8.4 & 2.97 & 1.41 & 26.3\% & 40.3\% \\
2020 & 1,097 & 312 & 10.7\% & 8.3\% & $-$2.4 & $-$1.31 & $-$0.77 & 37.1\% & 45.8\% \\
2021 & 713 & 177 & 3.1\% & 1.6\% & $-$1.5 & $-$0.71 & $-$0.34 & 23.0\% & 29.4\% \\
2022 & 1,169 & 203 & 0.9\% & 4.1\% & 3.2 & 1.69 & 1.19 & 24.8\% & 37.4\% \\
2023 & 1,122 & 201 & 2.4\% & 7.9\% & 5.5 & 2.93 & 1.90 & 25.8\% & 45.3\% \\
2024 & 851 & 213 & 3.2\% & 5.3\% & 2.0 & 0.99 & 0.74 & 26.2\% & 35.7\% \\
\multicolumn{10}{l}{\emph{By split}} \\
Train (2018--2022) & 4,094 & 873 & 4.6\% & 5.9\% & 1.3 & 1.33 & 0.74 & 27.7\% & 38.0\% \\
Validation (2023) & 1,122 & 201 & 2.4\% & 7.9\% & 5.5 & 2.93 & 1.90 & 25.8\% & 45.3\% \\
Test (2024) & 851 & 213 & 3.2\% & 5.3\% & 2.0 & 0.99 & 0.74 & 26.2\% & 35.7\% \\
\multicolumn{10}{l}{\emph{By 30-day average dollar volume (terciles)}} \\
ADDV tercile 1 (least liquid) & 2,103 & 336 & 1.8\% & 4.7\% & 3.0 & 1.97 & 1.13 & 22.0\% & 36.3\% \\
ADDV tercile 2 & 1,980 & 400 & 2.7\% & 2.9\% & 0.1 & 0.10 & 0.06 & 23.9\% & 28.2\% \\
ADDV tercile 3 (most liquid) & 1,984 & 551 & 7.7\% & 9.3\% & 1.6 & 1.21 & 0.73 & 36.0\% & 47.9\% \\
\multicolumn{10}{l}{\emph{By market capitalization}} \\
Market-cap tercile 1 (smallest) & 1,990 & 569 & 6.0\% & 6.6\% & 0.6 & 0.44 & 0.29 & 34.3\% & 40.2\% \\
Market-cap tercile 2 & 2,081 & 408 & 2.8\% & 6.6\% & 3.8 & 2.84 & 1.41 & 23.1\% & 35.3\% \\
Market-cap tercile 3 (largest) & 1,996 & 310 & 3.3\% & 4.7\% & 1.3 & 1.00 & 0.69 & 24.3\% & 40.6\% \\
Interior band \$60M--\$400M & 4,973 & 1,027 & 4.1\% & 5.6\% & 1.5 & 1.71 & 1.01 & 27.6\% & 38.7\% \\
Interior band \$100M--\$300M & 3,374 & 677 & 3.2\% & 4.5\% & 1.3 & 1.22 & 0.65 & 25.8\% & 35.2\% \\
\multicolumn{10}{l}{\emph{By industry}} \\
Non-biotech & 5,218 & 917 & 4.1\% & 4.4\% & 0.3 & 0.35 & 0.22 & 26.1\% & 33.3\% \\
Biotech / pharma & 849 & 370 & 3.8\% & 10.4\% & 6.7 & 4.00 & 2.65 & 33.8\% & 52.4\% \\
\multicolumn{10}{l}{\emph{By insider role (mutually exclusive)}} \\
CEO or CFO & 1,535 & 310 & 4.9\% & 6.3\% & 1.4 & 0.84 & 0.71 & 31.2\% & 40.3\% \\
Other officer & 679 & 151 & 6.1\% & 7.6\% & 1.5 & 0.64 & 0.47 & 30.8\% & 39.7\% \\
Director only & 2,771 & 482 & 4.0\% & 7.4\% & 3.5 & 2.69 & 2.16 & 25.6\% & 40.7\% \\
10\% owner (non-officer) & 960 & 284 & 1.3\% & 6.7\% & 5.5 & 2.93 & 2.45 & 22.4\% & 39.8\% \\
\multicolumn{10}{l}{\emph{By purchase history}} \\
Repeat purchaser (12 months) & 3,708 & 634 & 3.1\% & 6.3\% & 3.2 & 2.72 & 2.14 & 23.9\% & 38.3\% \\
First purchase in 12 months & 2,359 & 653 & 5.5\% & 5.9\% & 0.4 & 0.41 & 0.24 & 32.3\% & 39.2\% \\
\multicolumn{10}{l}{\emph{Issuer concentration}} \\
Excluding serial issuers ($\geq$ 50 lines) & 4,943 & 1,205 & 5.1\% & 6.6\% & 1.5 & 1.79 & 1.08 & 30.7\% & 39.7\% \\
Ticker-equal-weighted means (N = tickers) & 1,009 & 487 & 4.8\% & 5.8\% & 1.0 & 0.76 & 0.84 & 32.3\% & 37.3\% \\
\bottomrule


==> outputs/table_sample_stats_byyear.tex <==
2018 & 1,122 & 264 & 668 & 21.5\% & 1.8\% & 0.7\% & 47.7\% \\
2019 & 1,405 & 311 & 810 & 27.5\% & 4.9\% & 2.2\% & 42.8\% \\
2020 & 2,286 & 486 & 1,341 & 35.6\% & 7.8\% & 2.9\% & 39.7\% \\
2021 & 1,715 & 379 & 945 & 22.5\% & 2.5\% & 0.6\% & 38.6\% \\
2022 & 2,516 & 502 & 1,206 & 25.4\% & 1.4\% & 0.4\% & 30.4\% \\
2023 & 2,457 & 510 & 1,357 & 27.3\% & 2.9\% & 1.6\% & 20.9\% \\
2024 & 2,033 & 479 & 1,064 & 26.2\% & 3.3\% & 1.3\% & 14.4\% \\
\midrule
All & 13,534 & 1,192 & 4,809 & 27.1\% & 3.6\% & 1.3\% & 34.7\% \\
\bottomrule


==> outputs/table_sample_stats_car_dist.tex <==
$CAR_{[1,30]}$ (FF3, betas only), all years & 13,534 & 100.0\% & 3.6\% & 1.3\% & 21.5\% & $-$94\% & 474\% & $-$43.8\% & 71.5\% & 2.87 \\
$CAR_{[1,30]}$ (FF3, betas only), 2024 & 2,033 & 100.0\% & 3.3\% & 1.3\% & 21.7\% & $-$86\% & 164\% & $-$45.0\% & 83.6\% & 1.48 \\
$BHAR_{[1,30]}$ (FF3, betas only) & 13,534 & 100.0\% & 3.2\% & 0.1\% & 24.6\% & $-$80\% & 622\% & $-$39.2\% & 84.3\% & 5.30 \\
market-adjusted $CAR_{[1,30]}$ & 13,534 & 100.0\% & 2.8\% & 0.5\% & 22.0\% & $-$87\% & 471\% & $-$46.1\% & 72.7\% & 2.66 \\
$CAR_{[1,20]}$ (FF3, betas only) & 13,534 & 100.0\% & 3.2\% & 1.1\% & 17.3\% & $-$109\% & 199\% & $-$35.9\% & 60.6\% & 1.55 \\
$CAR_{[1,60]}$ (FF3, betas only) & 13,323 & 98.4\% & 4.6\% & 2.1\% & 31.0\% & $-$143\% & 467\% & $-$69.0\% & 105.0\% & 1.83 \\
$CAR_{[1,30]}$, next-day start for after-close filings & 13,534 & 100.0\% & 2.0\% & 0.2\% & 21.5\% & $-$86\% & 532\% & $-$45.2\% & 66.5\% & 3.67 \\
$CAR_{[1,30]}$, intercept-inclusive benchmark, all years & 13,534 & 100.0\% & 4.5\% & 2.1\% & 22.7\% & $-$103\% & 473\% & $-$45.5\% & 75.2\% & 2.53 \\
$CAR_{[1,30]}$, intercept-inclusive benchmark, 2024 & 2,033 & 100.0\% & 3.6\% & 1.6\% & 22.7\% & $-$73\% & 174\% & $-$45.8\% & 81.2\% & 1.53 \\
$BHAR_{[1,30]}$, intercept-inclusive benchmark & 13,534 & 100.0\% & 3.9\% & 0.8\% & 25.7\% & $-$110\% & 621\% & $-$43.1\% & 89.2\% & 4.70 \\
\bottomrule


==> outputs/table_sample_stats_car_tails.tex <==
$CAR_{[1,30]}$ (FF3, betas only), all years & 8.3\% & 3.1\% & 0.51\% & 27.1\% & 73rd & 26.4\% \\
$CAR_{[1,30]}$ (FF3, betas only), 2024 & 8.9\% & 4.1\% & 0.84\% & 26.2\% & 74th & 26.6\% \\
$BHAR_{[1,30]}$ (FF3, betas only) & 7.9\% & 2.9\% & 0.71\% & 24.3\% & 76th & 25.4\% \\
market-adjusted $CAR_{[1,30]}$ & 7.9\% & 4.0\% & 0.48\% & 26.5\% & 74th & 26.2\% \\
$CAR_{[1,20]}$ (FF3, betas only) & 5.9\% & 1.8\% & 0.25\% & 23.6\% & 76th & 22.1\% \\
$CAR_{[1,60]}$ (FF3, betas only) & 13.0\% & 7.8\% & 1.30\% & 33.7\% & 66th & 37.2\% \\
$CAR_{[1,30]}$, next-day start for after-close filings & 6.9\% & 3.7\% & 0.45\% & 24.2\% & 76th & 23.7\% \\
$CAR_{[1,30]}$, intercept-inclusive benchmark, all years & 9.6\% & 3.4\% & 0.54\% & 29.7\% & 70th & 29.0\% \\
$CAR_{[1,30]}$, intercept-inclusive benchmark, 2024 & 8.6\% & 4.4\% & 0.79\% & 27.8\% & 72nd & 26.6\% \\
$BHAR_{[1,30]}$, intercept-inclusive benchmark & 9.1\% & 3.4\% & 0.74\% & 27.0\% & 73rd & 27.6\% \\
\bottomrule


==> outputs/table_sample_stats_features_train.tex <==
\texttt{insider\_title\_score} & 9,044 & 2.4 & 1.4 & 1.0 & 1.0 & 2.0 & 5.0 & 5.0 & 0.0\% \\
\texttt{transaction\_value} & 9,044 & \$594k & \$11.4M & \$5k & \$9k & \$43k & \$412k & \$9.9M & 0.0\% \\
\texttt{is\_first\_purchase\_12m} & 9,044 & 0.399 & 0.490 & 0.000 & 0.000 & 0.000 & 1.000 & 1.000 & 0.0\% \\
\texttt{value\_vs\_avg\_ratio} & 5,427 & 2.67 & 31.06 & 0.01 & 0.19 & 0.83 & 2.88 & 24.09 & 40.0\% \\
\texttt{price\_deviation} & 9,044 & 0.015 & 0.105 & $-$0.246 & $-$0.062 & 0.004 & 0.096 & 0.464 & 0.0\% \\
\texttt{pct\_from\_52w\_high} & 9,044 & $-$0.426 & 0.244 & $-$0.915 & $-$0.775 & $-$0.417 & $-$0.105 & $-$0.017 & 0.0\% \\
\texttt{pct\_from\_52w\_low} & 9,044 & 0.663 & 2.206 & 0.003 & 0.040 & 0.250 & 1.388 & 6.973 & 0.0\% \\
\texttt{volatility\_30d} & 9,044 & 0.729 & 0.539 & 0.131 & 0.243 & 0.616 & 1.299 & 2.837 & 0.0\% \\
\texttt{return\_mtd} & 9,044 & $-$0.034 & 0.256 & $-$0.610 & $-$0.258 & $-$0.022 & 0.144 & 0.663 & 0.0\% \\
\texttt{market\_cap\_pit} & 9,044 & \$228.3M & \$125.2M & \$34.9M & \$76.2M & \$207.7M & \$419.6M & \$491.8M & 0.0\% \\
\texttt{addv\_30d} & 9,044 & \$3.0M & \$13.7M & \$208k & \$283k & \$898k & \$5.2M & \$34.6M & 0.0\% \\
\texttt{is\_biotech} & 9,044 & 0.149 & 0.356 & 0.000 & 0.000 & 0.000 & 1.000 & 1.000 & 0.0\% \\
\texttt{is\_ceo} & 9,044 & 0.182 & 0.386 & 0.000 & 0.000 & 0.000 & 1.000 & 1.000 & 0.0\% \\
\texttt{is\_cfo} & 9,044 & 0.068 & 0.251 & 0.000 & 0.000 & 0.000 & 0.000 & 1.000 & 0.0\% \\
\texttt{is\_other\_officer} & 9,044 & 0.225 & 0.418 & 0.000 & 0.000 & 0.000 & 1.000 & 1.000 & 0.0\% \\
\texttt{is\_director} & 9,044 & 0.529 & 0.499 & 0.000 & 0.000 & 1.000 & 1.000 & 1.000 & 0.0\% \\
\texttt{is\_10pct\_owner} & 9,044 & 0.219 & 0.414 & 0.000 & 0.000 & 0.000 & 1.000 & 1.000 & 0.0\% \\
\texttt{n\_prior\_purchases\_365d} & 9,044 & 3.5 & 7.4 & 0.0 & 0.0 & 1.0 & 10.0 & 38.0 & 0.0\% \\
\texttt{days\_since\_last\_purchase} & 6,234 & 145.9 & 245.3 & 1.0 & 2.0 & 46.0 & 440.0 & 1039.4 & 31.1\% \\
\texttt{n\_other\_insiders\_30d} & 9,044 & 1.3 & 2.1 & 0.0 & 0.0 & 1.0 & 4.0 & 10.0 & 0.0\% \\
\texttt{n\_purchases\_30d} & 9,044 & 1.8 & 3.2 & 0.0 & 0.0 & 1.0 & 5.0 & 15.6 & 0.0\% \\
\texttt{cmp\_routine} & 4,219 & 0.014 & 0.118 & 0.000 & 0.000 & 0.000 & 0.000 & 1.000 & 53.4\% \\
\texttt{filing\_lag\_days} & 9,044 & 2.6 & 5.3 & 0.0 & 0.0 & 2.0 & 4.0 & 21.0 & 0.0\% \\
\texttt{pct\_of\_holdings} & 9,040 & 0.17 & 0.55 & 0.00 & 0.00 & 0.05 & 0.50 & 1.00 & 0.0\% \\
\texttt{return\_5d} & 9,044 & $-$0.014 & 0.302 & $-$0.461 & $-$0.180 & $-$0.011 & 0.125 & 0.484 & 0.0\% \\
\texttt{return\_21d} & 9,044 & $-$0.044 & 0.548 & $-$0.691 & $-$0.343 & $-$0.045 & 0.201 & 0.897 & 0.0\% \\
\texttt{pre\_close} & 9,044 & 0.410 & 0.492 & 0.000 & 0.000 & 0.000 & 1.000 & 1.000 & 0.0\% \\
\bottomrule


==> outputs/table_sample_stats_funnel.tex <==
0 & OpenInsider purchase lines (raw scrape) & 0 & 101,093 & 6,390 \\
0b & trade\_type == 'P - Purchase' & 0 & 101,093 & 6,390 \\
1 & ticker cleaned and non-empty & 0 & 101,093 & 6,390 \\
2 & filing\_date in 2018-01-01..2024-12-31 and transaction\_date $\geq$ 2018-01-01 & 545 & 100,548 & 6,324 \\
3 & reporting lag 0 $\leq$ filing\_date - transaction\_date $\leq$ 90 calendar days & 1,727 & 98,821 & 6,230 \\
4 & transaction\_price $>$ 0, qty $>$ 0, transaction\_value $>$ 0 & 1,859 & 96,962 & 6,061 \\
5 & $|$value - price $\times$ qty$|$ $\leq$ 1\% of value & 3,459 & 93,503 & 5,957 \\
6 & transaction\_value $\geq$ \$5,000 & 17,046 & 76,457 & 5,826 \\
7 & duplicate lines (ticker, insider, trade date, price, qty, owned): keep earliest filing & 614 & 75,843 & 5,826 \\
8 & Yahoo panel coverage: ticker present and t0 = last trading day $\leq$ filing date exists & 26,322 & 49,521 & 3,395 \\
9a & $\geq$ 252 daily-return rows before t0 (253 price rows) for the FF3 estimation window & 4,235 & 45,286 & 3,182 \\
9b & $\geq$ 30 trading rows after t0 within the panel (full event window) & 0 & 45,286 & 3,182 \\
10a & a share count exists (SEC cover page filed $<$ t and $\leq$ 400 d old; else Jan-2026 snapshot) & 81 & 45,205 & 3,171 \\
10b & 30M $\leq$ market cap (close\_actual $\times$ SEC point-in-time shares) $\leq$ 500M & 20,177 & 25,028 & 1,724 \\
10c & 30M $\leq$ market cap $\leq$ 500M, rows on the snapshot fallback (no SEC observation) & 2,500 & 22,528 & 1,520 \\
10d & 30M $\leq$ market cap $\leq$ 500M, rows on the snapshot fallback (SEC observation $>$ 400 d old) & 2,452 & 20,076 & 1,444 \\
11 & ADDV (mean Volume $\times$ Close over the 30 trading rows ending t0, $\geq$ 20 obs) $>$ \$200,000 & 6,134 & 13,942 & 1,232 \\
12 & close\_actual(t0) / transaction\_price within [0.5, 2] (symmetric band; corporate-action mismatches) & 203 & 13,739 & 1,216 \\
12b & ticker-year price basis: median close\_actual/Form-4 price on lag$\leq$2 lines ($\geq$3, full scrape) in [0.75, 1.33] & 192 & 13,547 & 1,193 \\
13a & CAR\_30 computable (no estimation failure) & 0 & 13,547 & 1,193 \\
13b & CAR\_30 $\geq$ -1 (outlier screen; primary benchmark) & 9 & 13,538 & 1,192 \\
13c & no one-day price ratio $\geq$ 8 or $\leq$ 1/8 inside the event window (unrecorded corporate action) & 4 & 13,534 & 1,192 \\
\bottomrule

